Exploring the origins of mega radio halos

We present a first attempt to investigate the origin of radio-emitting electrons in the newly discovered class of mega radio halos in clusters of galaxies. We study the evolution of relativistic electrons accreted by the external regions of a simulated cluster of galaxies at high resolution, including the effect of radiative losses and turbulent reacceleration acting on relativistic electrons. We conclude that turbulent reacceleration induced by structure formation, if sufficiently prolonged, has the potential to produce a large reservoir of radio-emitting electrons in the large regions illuminated by mega radio halos observed by LOFAR.

==> 0_referee_report_with_replies.tex <==
We thank our Reviewer for his feedback on our work: it turned out to be extremely helpful.
In this revised version, we took into account all suggestions, and introduced longer and more detailed explanations of several crucial points. This resulted into a longer manuscript, including 4 new plots (arranged in new Fig. 3 and 6). 
All important modifications introduced in the manuscript are marked in boldface. Here below is our detailed list of answers to our Reviewer's comments.
We hope that this work can now be considered for publication.
Best regards
L. Beduzzi (on behalf of all coauthors).



=================================================

R:--- It is stressed on p. 4, and re-stressed on p. 6, that a fundamental finding (even a surprise?) here is that CR electrons live longer than expected (it is not entirely clear by whom this was expected, or on what grounds, maybe a reference would help?). 

A: This is indeed a key result of our paper, and in order to better show how this may revise the more classical estimates of the lifetime of radio emitting electrons in the ICM, we added a longer dedicated discussion in Sec.4, as well as a three panel Figure (new Fig. 6), which should best illustrate our result in a concise way. 


R: On p. 4, and then 5, this is explained by a balance of re-acceleration and loss time scales, gleaned from numerical measurements. Can some useful twiddle estimate be made here? If I assume such a balance, can I predict this result analytically? What would this imply for various scalings? Importantly, what would this imply for how fine-tuned this result is --- what would break it and how sensitive is the viability of such a balance to theoretical assumptions and numerical choices? I am not demanding a quantitative theory, just a back-of-a-napkin theoretical scoping out to match the numerical one reported here.

A: Similar as before: the new Fig.6 illustrates how the classical picture of the distribution of CR lifetimes in a cluster is changed if we include the new view of turbulent re-acceleration highlighted by our analysis. This has also led to a longer concluding discussion, in Sec.4.  

R:
--- Another important numerical finding seems to be that the CR electrons in MegaRH have been inside the Classical RH already, rather then accreting from outside. Again, can some useful twiddle estimate be made here, say, how long does a CR electron stay confined and so does it make sense to think of the MegaRH as a kind of atmosphere/corona through which these electrons are evaporating out? Does the size of the MegaRH make sense in that context?

A: We produced a new figure (Fig.3) to strengthen this point: it gives the evolution with time of the median distance of the families of tracers from the cluster centre, and it shows that the two family were almost at the same distance at all times, with the exception of the latest 1-2 Gyrs. 


R:--- Perhaps some brief discussion of why the Brunetti-Lazarian re-acceleration scheme should be used rather than something else? I know this is referred to previous literature, but for a busy astronomer who is prepared to read just this, can you make an elevator pitch for why this is the right physics to invoke (beyond just "we use it and it works fine").
A: We added a longer discussion of this in Sec.2.1 


R:
--- There is a reference to scale L in eq. 1 not mattering in a Kolmogorov V^3/L = const situation. Great, but is Kolmogorov incompressible turbulence actually what you have in there? What are the Mach numbers? Is there a spectrum of motions that at all resembles K41?
A: We added a longer comment on this at the end of Sec.2, in which we referred to our previous works on the issue. 



R: --- A significant model-dependent aspect seems to be the question of how CR electrons might diffuse and, therefore, whether the whole particle-tracking scheme followed here is sensible. Footnote 1 quotes a CR diffusion scale of < 100 pc but gives no explanation of how this obtained. Can you explain what is assumed and assess how sensitive your results are to that? There is a huge literature on CR confinement, both physics and modelling, so it would be useful to connect to that.
A: We addressed this issue, with a longer explanation and line showing the relative value of CR diffusion compared to other timescales, in Sec.4 and Fig.6.


Some minor issues:

R: On p. 2, they mention scaling up the organically created magnetic fields --- but they don't explain how, by how much, how these scaled-up fields are maintained etc. In footnote 1, there is an intimation that they are on microGauss level, and one can see that also in Fig 2a, but there's no detail. A bit more info would help.
A: We added a longer explanation about this procedure at the end of Sec.2. 



R: 
At the bottom of the left column of p. 2, there is an incomplete sentence: "The distribution of particles was created by sampling a fixed gas mass resolution of..." ---???
A: We fixed this in the revised draft, thanks.

R:
p. 5 major mergers ---> major merger; gas always keep ---> gas always keeps
A: done 


